Dark Energy Survey Year 3: Blue Shear

Modeling the intrinsic alignment (IA) of galaxies poses a challenge to weak lensing analyses. The Dark Energy Survey is expected to be less impacted by IA when limited to blue, star-forming galaxies. The cosmological parameter constraints from this blue cosmic shear sample are stable to IA model choice, unlike passive galaxies in the full DES Y3 sample, the goodness-of-fit is improved and the $\Omega_{m}$ and $S_8$ better agree with the cosmic microwave background. Mitigating IA with sample selection, instead of flexible model choices, can reduce uncertainty in $S_8$ by a factor of 1.5.

==> cosmo_table.tex <==
\begin{tabular}{ccccccccccccc}
\hline
\hline
\\ Model & $S_{8, {\rm mean}}$ & $\Omega_{{\rm m, mean}} $ & \makecell{Evid.\\Ratio} & $\chi_{\mathrm{min}}^2$  & $\chi_{\mathrm{\textsc{red}}}^2$ & $\delta S_8$ & $\delta \Omega_m$ & $\sqrt{\delta S_8^2 + \delta \Omega_m^2}$\\
\hline
 \textsc{full} NLA ($a_1$) & $ 0.810^{+0.015}_{-0.020} $ & $0.253^{+0.029}_{-0.043} $ & {1.00} & {476.6} & {1.2} & {0.75} & {1.60} & {1.77} \\ 
  \textsc{full} NLA-$z$ ($a_1,\eta_1$) & $ 0.808^{+0.022}_{-0.019} $ & $0.243^{+0.031}_{-0.044} $ & {1.75} & {476.8} & {1.2} & {0.75} & {1.83} & {1.97} \\ 
  \textsc{full} TATT & $ 0.784^{+0.031}_{-0.022} $ & $0.253^{+0.029}_{-0.047} $ & {0.88} & {470.4} & {1.2} & {1.33} & {1.53} & {2.03} \\ 
  \textbf{\textsc{full} No IA} & $ 0.810^{+0.015}_{-0.018} $ & $0.255^{+0.031}_{-0.040} $ & {12.91} & {477.2} & {1.2} & {0.77} & {1.61} & {1.78} \\ 
  \textsc{full} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.791^{+0.022}_{-0.017} $ & $0.268^{+0.041}_{-0.053} $ &  & {356.4} & {1.3} & {1.36} & {0.92} & {1.64} \\ 
  \textsc{full} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.776^{+0.031}_{-0.025} $ & $0.268^{+0.036}_{-0.045} $ &  & {350.8} & {1.3} & {1.51} & {1.06} & {1.84} \\ 
 \hline 
  \textsc{red} NLA ($a_1$) & $ 0.821^{+0.020}_{-0.022} $ & $0.221^{+0.019}_{-0.046} $ & {1.00} & {498.4} & {1.3} & {0.28} & {2.33} & {2.34} \\ 
  \textsc{red} NLA-$z$ ($a_1,\eta_1$) & $ 0.821^{+0.022}_{-0.022} $ & $0.220^{+0.019}_{-0.045} $ & {1.07} & {499.7} & {1.3} & {0.26} & {2.34} & {2.36} \\ 
  \textsc{red} TATT & $ 0.750^{+0.045}_{-0.035} $ & $0.224^{+0.021}_{-0.052} $ & {5.53} & {491.8} & {1.2} & {1.71} & {1.93} & {2.58} \\ 
  \textbf{\textsc{red} No IA} & $ 0.818^{+0.019}_{-0.020} $ & $0.210^{+0.016}_{-0.039} $ & {7.38} & {498.4} & {1.3} & {0.39} & {3.02} & {3.05} \\ 
  \textsc{red} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.794^{+0.026}_{-0.026} $ & $0.237^{+0.023}_{-0.062} $ &  & {360.0} & {1.3} & {1.04} & {1.46} & {1.79} \\ 
  \textsc{red} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.757^{+0.051}_{-0.031} $ & $0.237^{+0.023}_{-0.056} $ &  & {358.3} & {1.3} & {1.45} & {1.54} & {2.12} \\ 
 \hline 
  \textsc{blue} NLA ($a_1$) & $ 0.821^{+0.021}_{-0.021} $ & $0.264^{+0.030}_{-0.062} $ & {1.00} & {442.8} & {1.1} & {0.25} & {0.98} & {1.01} \\ 
  \textsc{blue} NLA-$z$ ($a_1,\eta_1$) & $ 0.818^{+0.024}_{-0.024} $ & $0.263^{+0.031}_{-0.066} $ & {1.56} & {443.4} & {1.1} & {0.34} & {0.92} & {0.98} \\ 
  \textsc{blue} TATT & $ 0.795^{+0.047}_{-0.027} $ & $0.260^{+0.035}_{-0.057} $ & {0.79} & {440.0} & {1.1} & {0.73} & {1.11} & {1.32} \\ 
  \textbf{\textsc{blue} No IA} & $ 0.822^{+0.017}_{-0.019} $ & $0.269^{+0.035}_{-0.051} $ & {10.23} & {443.0} & {1.1} & {0.23} & {0.97} & {1.00} \\ 
  \textsc{blue} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.770^{+0.055}_{-0.026} $ & $0.273^{+0.046}_{-0.075} $ &  & {305.0} & {1.1} & {1.17} & {0.64} & {1.33} \\ 
  \textsc{blue} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.755^{+0.065}_{-0.032} $ & $0.286^{+0.046}_{-0.066} $ &  & {297.2} & {1.1} & {1.22} & {0.47} & {1.31} \\ 
 
\hline
\end{tabular}

==> full_table.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table*}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccc}
\hline
\hline
\\ Model & $S_{\rm{{8, mean}}$ & $\Omega_{m, mean} $ & \makecell{Evid.\\Ratio} & $\chi_{\mathrm{min}}^2$  & $\chi_{\mathrm{\textsc{red}}}^2$ & $p$ & $\delta S_8$ & $\delta \Omega_m$ & $\sqrt{\delta S_8^2 + \delta \Omega_m^2}$\\
\hline
 \textsc{full} NLA ($a_1$) & $ 0.810^{+0.015}_{-0.020} $ & $0.253^{+0.029}_{-0.043} $& {1.000} & {476.56} & {1.21} & {0.0030} & {0.754} & {1.603} & {1.772} \\ 
  \textsc{full} NLA ($a_1,\eta_1$) & $ 0.808^{+0.022}_{-0.019} $ & $0.243^{+0.031}_{-0.044} $& {1.748} & {476.81} & {1.21} & {0.0029} & {0.748} & {1.827} & {1.974} \\ 
  \textsc{full} TATT & $ 0.784^{+0.031}_{-0.022} $ & $0.253^{+0.029}_{-0.047} $& {0.883} & {470.41} & {1.19} & {0.0053} & {1.332} & {1.526} & {2.025} \\ 
  \textsc{full} TATT ($b_{ta} = 1.0$) & $ 0.787^{+0.032}_{-0.023} $ & $0.249^{+0.032}_{-0.045} $& {0.993} & {470.32} & {1.19} & {0.0054} & {1.230} & {1.584} & {2.006} \\ 
  \textsc{full} No IA & $ 0.810^{+0.015}_{-0.018} $ & $0.255^{+0.031}_{-0.040} $& {12.911} & {477.16} & {1.21} & {0.0028} & {0.771} & {1.607} & {1.782} \\ 
  \textsc{full} NLA, No AGN Feedback & $ 0.781^{+0.016}_{-0.012} $ & $0.265^{+0.037}_{-0.049} $& {0.233} & {479.89} & {1.21} & {0.0022} & {2.032} & {1.083} & {2.303} \\ 
  \textsc{full} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.791^{+0.022}_{-0.017} $ & $0.268^{+0.041}_{-0.053} $& {1.000} & {356.41} & {1.33} & {0.0002} & {1.360} & {0.922} & {1.643} \\ 
  \textsc{full} No IA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.792^{+0.016}_{-0.016} $ & $0.269^{+0.032}_{-0.051} $& {8.667} & {356.33} & {1.33} & {0.0002} & {1.549} & {0.985} & {1.836} \\ 
  \textsc{full} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.776^{+0.031}_{-0.025} $ & $0.268^{+0.036}_{-0.045} $& {0.679} & {350.80} & {1.31} & {0.0005} & {1.507} & {1.062} & {1.844} \\ 
 \hline 
  \textsc{red} NLA ($a_1$) & $ 0.821^{+0.020}_{-0.022} $ & $0.221^{+0.019}_{-0.046} $& {1.000} & {498.43} & {1.26} & {0.0003} & {0.281} & {2.327} & {2.344} \\ 
  \textsc{red} NLA ($a_1,\eta_1$) & $ 0.821^{+0.022}_{-0.022} $ & $0.220^{+0.019}_{-0.045} $& {1.072} & {499.74} & {1.27} & {0.0003} & {0.256} & {2.344} & {2.358} \\ 
  \textsc{red} TATT & $ 0.750^{+0.045}_{-0.035} $ & $0.224^{+0.021}_{-0.052} $& {5.530} & {491.78} & {1.25} & {0.0006} & {1.706} & {1.932} & {2.577} \\ 
  \textsc{red} TATT ($b_{ta} = 1.0$) & $ 0.745^{+0.047}_{-0.034} $ & $0.223^{+0.023}_{-0.052} $& {4.905} & {490.83} & {1.24} & {0.0007} & {1.818} & {2.113} & {2.788} \\ 
  \textsc{red} No IA & $ 0.818^{+0.019}_{-0.020} $ & $0.210^{+0.016}_{-0.039} $& {7.382} & {498.42} & {1.26} & {0.0003} & {0.389} & {3.020} & {3.045} \\ 
  \textsc{red} NLA, No AGN Feedback & $ 0.800^{+0.017}_{-0.015} $ & $0.220^{+0.018}_{-0.045} $& {1.206} & {500.24} & {1.27} & {0.0003} & {1.157} & {2.354} & {2.623} \\ 
  \textsc{red} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.794^{+0.026}_{-0.026} $ & $0.237^{+0.023}_{-0.062} $& {1.000} & {360.02} & {1.34} & {0.0001} & {1.043} & {1.461} & {1.795} \\ 
  \textsc{red} No IA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.789^{+0.024}_{-0.024} $ & $0.228^{+0.021}_{-0.054} $& {6.814} & {359.69} & {1.34} & {0.0002} & {1.390} & {1.843} & {2.308} \\ 
  \textsc{red} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.757^{+0.051}_{-0.031} $ & $0.237^{+0.023}_{-0.056} $& {0.398} & {358.27} & {1.34} & {0.0002} & {1.451} & {1.541} & {2.117} \\ 
 \hline 
  \textsc{blue} NLA ($a_1$) & $ 0.821^{+0.021}_{-0.021} $ & $0.264^{+0.030}_{-0.062} $& {1.000} & {442.78} & {1.12} & {0.0485} & {0.250} & {0.979} & {1.010} \\ 
  \textsc{blue} NLA ($a_1,\eta_1$) & $ 0.818^{+0.024}_{-0.024} $ & $0.263^{+0.031}_{-0.066} $& {1.563} & {443.38} & {1.12} & {0.0465} & {0.335} & {0.923} & {0.982} \\ 
  \textsc{blue} TATT & $ 0.795^{+0.047}_{-0.027} $ & $0.260^{+0.035}_{-0.057} $& {0.787} & {440.03} & {1.11} & {0.0584} & {0.730} & {1.106} & {1.325} \\ 
  \textsc{blue} TATT ($b_{ta} = 1.0$) & $ 0.791^{+0.050}_{-0.027} $ & $0.265^{+0.033}_{-0.060} $& {0.759} & {438.81} & {1.11} & {0.0633} & {0.794} & {0.930} & {1.222} \\ 
  \textsc{blue} No IA & $ 0.822^{+0.017}_{-0.019} $ & $0.269^{+0.035}_{-0.051} $& {10.229} & {442.96} & {1.12} & {0.0479} & {0.231} & {0.969} & {0.996} \\ 
  \textsc{blue} NLA, No AGN Feedback & $ 0.794^{+0.031}_{-0.016} $ & $0.270^{+0.040}_{-0.063} $& {1.133} & {443.63} & {1.12} & {0.0458} & {1.062} & {0.772} & {1.313} \\ 
  \textsc{blue} NLA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.770^{+0.055}_{-0.026} $ & $0.273^{+0.046}_{-0.075} $& {1.000} & {304.97} & {1.14} & {0.0597} & {1.169} & {0.635} & {1.330} \\ 
  \textsc{blue} No IA, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.795^{+0.022}_{-0.021} $ & $0.294^{+0.042}_{-0.060} $& {8.053} & {306.27} & {1.14} & {0.0538} & {1.241} & {0.364} & {1.293} \\ 
  \textsc{blue} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.755^{+0.065}_{-0.032} $ & $0.286^{+0.046}_{-0.066} $& {2.095} & {297.21} & {1.11} & {0.1062} & {1.218} & {0.474} & {1.307} \\ 
 
\hline
\end{tabular}
}

\caption{Statistics for the comprehensive suite of Markov Chain Monte Carlo (MCMC) chains run with variations in model choice and sample of galaxies for cosmic shear. \note{This table is in the process of being updated with final chains, and the $\chi^2$ are artificially high from an older covariance matrix. It will be finalized by submission.}}
\label{tab:full_table}
\end{table*}

\setlength{\mytabcolsep}{\tabcolsep} %restore original table formatting

\begin{figure*}
    \includegraphics[width=0.68\textwidth]{figures/data_s8_summary.pdf}
    \hspace{3pt}
    \includegraphics[width=0.288\textwidth]{figures/data_om_summary.pdf}
    \caption{Summary statistics for each cosmological model fit, with the DES Y3 $\Lambda$CDM-Optimized result in shaded gray, and the \textit{Planck} results \cite{EfstathiouGratton:2021} in shaded orange. The 68\% confidence regions (1-$\sigma$) are reported for each model fit. \note{Similarly, this figure will be updated with final chains, though results do not change significantly.}}
    \label{fig:datasummary}
\end{figure*}

==> journal_defs.tex <==
%\let\jnl@style=\rmfamily 
%\def\rmfamily#1{{\jnl@style#1}}% 
\newcommand\aj{\rmfamily{AJ}}%        % Astronomical Journal 
\newcommand\araa{\rmfamily{ARA\&A}}%  % Annual Review of Astron and Astrophys 
%\newcommand\apj{\rmfamily{ApJ}}%    % Astrophysical Journal 
\newcommand\apjl{\rmfamily{ApJL}}%     % Astrophysical Journal, Letters 
\newcommand\apjs{\rmfamily{ApJS}}%    % Astrophysical Journal, Supplement 
%\newcommand\ao{\rmfamily{Appl.~Opt.}}%   % Applied Optics 
\newcommand\apss{\rmfamily{Ap\&SS}}%  % Astrophysics and Space Science 
\newcommand\aap{\rmfamily{A\&A}}%     % Astronomy and Astrophysics 
\newcommand\aapr{\rmfamily{A\&A~Rev.}}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{\rmfamily{A\&AS}}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{\rmfamily{AZh}}%       % Astronomicheskii Zhurnal 
\newcommand\baas{\rmfamily{BAAS}}%     % Bulletin of the AAS 
\newcommand\icarus{\rmfamily{Icarus}}% % Icarus
\newcommand\jrasc{\rmfamily{JRASC}}%   % Journal of the RAS of Canada 
\newcommand\memras{\rmfamily{MmRAS}}%  % Memoirs of the RAS 
\newcommand\mnras{\rmfamily{MNRAS}}%   % Monthly Notices of the RAS 
%\newcommand\pra{\rmfamily{Phys.~Rev.~A}}% % Physical Review A: General Physics 
%\newcommand\prb{\rmfamily{Phys.~Rev.~B}}% % Physical Review B: Solid State 
%\newcommand\prc{\rmfamily{Phys.~Rev.~C}}% % Physical Review C 
%\newcommand\prd{\rmfamily{Phys.~Rev.~D}}% % Physical Review D 
%\newcommand\pre{\rmfamily{Phys.~Rev.~E}}% % Physical Review E 
%\newcommand\prl{\rmfamily{Phys.~Rev.~Lett.}}% % Physical Review Letters 
\newcommand\pasp{\rmfamily{PASP}}%     % Publications of the ASP 
\newcommand\pasj{\rmfamily{PASJ}}%     % Publications of the ASJ 
\newcommand\qjras{\rmfamily{QJRAS}}%   % Quarterly Journal of the RAS 
\newcommand\skytel{\rmfamily{S\&T}}%   % Sky and Telescope 
\newcommand\solphys{\rmfamily{Sol.~Phys.}}% % Solar Physics 
\newcommand\sovast{\rmfamily{Soviet~Ast.}}% % Soviet Astronomy 
\newcommand\ssr{\rmfamily{Space~Sci.~Rev.}}% % Space Science Reviews 
\newcommand\zap{\rmfamily{ZAp}}%       % Zeitschrift fuer Astrophysik 
%\newcommand\nat{\rmfamily{Nature}}%  % Nature 
\newcommand\iaucirc{\rmfamily{IAU~Circ.}}% % IAU Cirulars 
\newcommand\aplett{\rmfamily{Astrophys.~Lett.}}%  % Astrophysics Letters 
\newcommand\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.}}% % Astrophysics Space Physics Research 
\newcommand\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands}}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{\rmfamily{Fund.~Cosmic~Phys.}}%   % Fundamental Cosmic Physics 
\newcommand\gca{\rmfamily{Geochim.~Cosmochim.~Acta}}% % Geochimica Cosmochimica Acta 
\newcommand\grl{\rmfamily{Geophys.~Res.~Lett.}}%  % Geophysics Research Letters 
%\newcommand\jcp{\rmfamily{J.~Chem.~Phys.}}%     % Journal of Chemical Physics 
\newcommand\jgr{\rmfamily{J.~Geophys.~Res.}}%     % Journal of Geophysics Research 
\newcommand\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.}}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana}}% % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{\rmfamily{Nucl.~Phys.~A}}%     % Nuclear Physics A 
\newcommand\physrep{\rmfamily{Phys.~Rep.}}%       % Physics Reports 
\newcommand\physscr{\rmfamily{Phys.~Scr}}%        % Physica Scripta 
\newcommand\planss{\rmfamily{Planet.~Space~Sci.}}%  % Planetary Space Science 
\newcommand\procspie{\rmfamily{Proc.~SPIE}}%      % Proceedings of the SPIE 

\newcommand\actaa{\rmfamily{Acta Astron.}}%  % Acta Astronomica
\newcommand\caa{\rmfamily{Chinese Astron. Astrophys.}}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\rmfamily{Chinese J. Astron. Astrophys.}}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{\rmfamily{J. Cosmology Astropart. Phys.}}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{\rmfamily{New A}}%  % New Astronomy
\newcommand\nar{\rmfamily{New A Rev.}}%  % New Astronomy Review
\newcommand\pasa{\rmfamily{PASA}}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{\rmfamily{Rev. Mexicana Astron. Astrofis.}}%  % Revista Mexicana de Astronomia y Astrofisica

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

==> map_table.tex <==
\begin{table*}
\resizebox{\textwidth}{!}{\begin{tabular}{ccccccccccccccc}
\hline
\hline
\\ Model & $S_{\rm{8, mean}}$ & $\Omega_{\rm{m, mean}} $ & $S_{\rm{8, MAP}}$ & $\Omega_{\rm{ m, MAP}} $ &\makecell{Evid.\\Ratio} & $\chi_{\mathrm{min}}^2$  & $\chi_{\mathrm{red}}^2$ & $\delta S_8$ & $\delta \Omega_m$ & $\sqrt{\delta S_8^2 + \delta \Omega_m^2}$\\
\hline
 \textsc{full} TATT, Y3 Scale Cuts\textsuperscript{\textdagger} & $ 0.774^{+0.033}_{-0.024} $ & $0.273^{+0.035}_{-0.048} $& $ 0.778 $ & $0.319$ & & {351.0} & {1.3} & {1.58} & {0.92} & {1.83} \\ 
  \textsc{red} TATT & $ 0.750^{+0.046}_{-0.038} $ & $0.225^{+0.025}_{-0.049} $& $ 0.743 $ & $0.179$ & & {492.2} & {1.2} & {1.65} & {2.09} & {2.66} \\ 
  \textbf{\textsc{blue} No IA} & $ 0.821^{+0.018}_{-0.020} $ & $0.273^{+0.035}_{-0.056} $& $ 0.815 $ & $0.267$ & & {444.2} & {1.1} & {0.25} & {0.84} & {0.88} \\ 
 
\hline
\end{tabular}}
\end{table*}

==> multinest_s8-om.tex <==
    \begin{subfigure}[t]{0.32\textwidth}     
    \includegraphics[width=1.02\textwidth]{figures/s8-om-full_nla1.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}       
    \includegraphics[width=1.02\textwidth]{figures/s8-om-red_nla1.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}       
    \includegraphics[width=1.02\textwidth]{figures/s8-om-blue_nla1.pdf}
    \end{subfigure}

==> polychord_scalecut_s8-om.tex <==
    \begin{subfigure}[t]{0.32\textwidth}     
    \includegraphics[width=1.02\textwidth]{figures/s8-om-full-poly-y3sc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}       
    \includegraphics[width=1.02\textwidth]{figures/s8-om-red-poly-y3sc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}       
    \includegraphics[width=1.02\textwidth]{figures/s8-om-blue-poly-y3sc.pdf}
    \end{subfigure}

